Asynchronous Distributed Optimization with Redundancy in Cost Functions

This paper considers the problem of asynchronous distributed multi-agent optimization on server-based system architecture. In this problem, each agent has a local cost, and the goal for the agents is to collectively find a minimum of their aggregate cost. A standard algorithm to solve this problem is the iterative distributed gradient-descent (DGD) method being implemented collaboratively by the server and the agents. In the synchronous setting, the algorithm proceeds from one iteration to the next only after all the agents complete their expected communication with the server. However, such synchrony can be expensive and even infeasible in real-world applications. We show that waiting for all the agents is unnecessary in many applications of distributed optimization, including distributed machine learning, due to redundancy in the cost functions (or {\em data}). Specifically, we consider a generic notion of redundancy named $(r,\epsilon)$-redundancy implying solvability of the original multi-agent optimization problem with $\epsilon$ accuracy, despite the removal of up to $r$ (out of total $n$) agents from the system. We present an asynchronous DGD algorithm where in each iteration the server only waits for (any) $n-r$ agents, instead of all the $n$ agents. Assuming $(r,\epsilon)$-redundancy, we show that our asynchronous algorithm converges to an approximate solution with error that is linear in $\epsilon$ and $r$. Moreover, we also present a generalization of our algorithm to tolerate some Byzantine faulty agents in the system. Finally, we demonstrate the improved communication efficiency of our algorithm through experiments on MNIST and Fashion-MNIST using the benchmark neural network LeNet.

==> asynchrony.tex <==
\section{Exploiting Redundancy for Asynchronous Distributed Optimization}
\label{sec:redundancy}

We consider two cases of redundancy in the cost functions; (i) the special case of $(r,0)$-redundancy, or exact redundancy (in Section \ref{sec:exact-redundancy}), and (ii) the general $(r,\epsilon)$-redundancy, or approximate redundancy (in Section \ref{sec:approx-redundancy}).

\subsection{Exact Redundancy}
\label{sec:exact-redundancy}

In this section, we provide convergence analysis of our algorithm given that the cost functions of agents satisfies $(r,0)$-redundancy. Note that the special case of $(r,0)$-redundancy %can also be written as the following $r$-redundancy:
is equivalent to the $r$-redundancy property defined as follows.

\begin{definition}[$r$-redundancy]
    \label{def:redundancy}
    For any two sets $S$ and $T$, each containing at least $n-r$ agents, 
    \begin{equation}
        \arg\min_x\sum_{j\in S}Q_j(x)=\arg\min_x\sum_{j\in T}Q_j(x).
        \label{eqn:redundancy}
    \end{equation}
\end{definition}
\noindent Intuitively, all sets of more than $n-r$ agents have their aggregated cost functions minimize at the same set of points. 

From now on, we use $[n]$ as a shorthand for the set $\{1,...,n\}$. Suppose the cost function for agent $i$ is $Q_i(x)$. We first introduce some assumptions on the cost functions that are necessary for our analysis.

\begin{assumption}
    \label{assum:lipschitz}
    For each $i$, the function $Q_i(x)$ is $\mu$-Lipschitz smooth, i.e., $\forall x, x'\in\mathbb{R}^d$, 
    \begin{equation}
        \norm{\nabla Q_i(x)-\nabla Q_i(x')}\leq\mu\norm{x-x'}.
    \end{equation}
\end{assumption}

\begin{assumption}
    \label{assum:strongly-convex}
    For any set $S\subset[n]$, we define the average cost function to be $\displaystyle Q_S(x)=\frac{1}{\mnorm{S}}\sum_{j\in S}Q_j(x)$. We assume that $Q_S(x)$ is $\gamma$-strongly convex for any $S$ subject to $\mnorm{S}\geq n-r$, i.e., $\forall x, x'\in\mathbb{R}^d$, 
    \begin{equation}
        \iprod{\nabla Q_S(x)-\nabla Q_S(x')}{x-x'}\geq\gamma\norm{x-x'}^2.
    \end{equation}
\end{assumption}

Given Assumption~\ref{assum:strongly-convex}, there is only one minimum point for any $S$, $\mnorm{S}\geq n-r$. Let us define $ x^*=\arg\min_x\sum_{j\in[n]}Q_j(x)$.
Thus, $x^*$ is the unique minimum point for the aggregated cost functions of all the agents. We assume that (recall that $\W$ is used in (\ref{eqn:update}))
\begin{equation}
    \label{eqn:existence-exact}
    x^*\in \W.
\end{equation}

The following is a corollary of the previous assumptions.

\begin{lemma}
\label{lemma:minimum}
Under Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex}, $\nabla Q_j(x^*)=0$ for all $j\in[n]$, if the cost functions of all agents satisfies $r$-redundancy property.
\end{lemma}

\begin{proof}
By Definition~\ref{def:redundancy}, the minimum point $x^*=\arg\min_x\sum_{i\in[n]}Q_i(x)$ also satisfies $x^*=\arg\min_x\sum_{i\in S}Q_i(x)$, for any $\mnorm{S}\geq n-r$. 

%Consider any set $T$ with $\mnorm{T}=n-r+1$ and $S\subsetneq T$ with $\mnorm{S}=n-r$. Let $j$ be the agent in $T$ that is not in $S$; $S=T-\{j\}$. 
Consider any set $S$ with $\mnorm{S}=n-r$ and any agent $j\not\in S$. Let $T=S\cup\{j\}$.
$S$ and $T$ satisfy (\ref{eqn:redundancy}), so 
\begin{equation}
    \sum_{i\in S}\nabla Q_i(x^*)=\sum_{i\in T}\nabla Q_i(x^*) = 0.
\end{equation}
Note that
\begin{equation}
    \sum_{i\in T}\nabla Q_i(x) = \sum_{i\in S}\nabla Q_i(x) + \nabla Q_j(x)
\end{equation}
Combine the two equations together, we have
\begin{equation}
    \nabla Q_j(x) = 0.
\end{equation}
Notice that the choice of $S$, $T$ and $j$ are arbitrary. Therefore, $\nabla Q_i(x^*)=0$, $\forall i\in[n]$.
\end{proof}

With $r$-redundancy, our algorithm can output $x^*$, the minimum point of the aggregation of cost functions of all the agents. To prove our main claim in this section, we will need the following lemma. 

Let us first define a generalized notation of gradient aggregation rule $\mathsf{GradAgg}:\R^{d\times n}\rightarrow\R^d$, a function mapping $n$ gradients to a $d$-dimensional vector. Under this notation, the iterative update of estimates in any aggregation-based algorithm can be written as
\begin{equation}
    x^{t+1}=\left[x^t-\eta_t\mathsf{GradAgg}\left(\nabla Q_1(x^t), ..., \nabla Q_n(x^t)\right)\right]_\W,
    \label{eqn:update-general}
\end{equation}
where for our algorithm, recall \eqref{eqn:update}, the gradient aggregation rule
\begin{equation}
    \mathsf{GradAgg}\left(\nabla Q_1(x^t), ..., \nabla Q_n(x^t)\right)=\sum_{j\in{S^t}}\nabla Q_j(x^t)
    \label{eqn:aggregation-rule}
\end{equation}
for all iteration $t$. Recall that although all $n$ gradients are formally mentioned in the aggregation rule, only those in $S^t$ are actually used, and in practice the algorithm doesn't need to wait for all $n$ gradients. With this notation, we state the lemma:

\begin{lemma}
    \label{lemma:bound}
    Consider the general iterative update rule (\ref{eqn:update-general}). Let $\eta_t$ satisfy
    \begin{equation}
        \sum_{t=0}^\infty\eta_t=\infty~\textrm{ and }~\sum_{t=0}^\infty\eta_t^2<\infty.
    \end{equation}
    For any given gradient aggregation rule $\mathsf{GradAgg}\left(\nabla Q_1(x^t), ..., \nabla Q_n(x^t)\right)$, if there exists $\M<\infty$ such that
    \begin{equation}
        \norm{\mathsf{GradAgg}\left(\nabla Q_1(x^t), ..., \nabla Q_n(x^t)\right)}\leq\M
        \label{eqn:bounded-aggregator-norm}
    \end{equation} for all $t$, and there exists $\D^*\in\left[0,\max_{x\in\W}\norm{x-x^*}\right)$ and $\xi>0$ such that when $\norm{x^t-x^*}\geq\D^*$,
    \begin{equation}
        \phi_t\triangleq\iprod{x^t-x^*}{\mathsf{GradAgg}\left(\nabla Q_1(x^t), ..., \nabla Q_n(x^t)\right)}\geq\xi,~
        \label{eqn:phi-def}
    \end{equation}
    we have $\lim_{t\rightarrow\infty}\norm{x^t-x^*}\leq\D^*$.
\end{lemma}
Note that the values of $\D^*$ and $\xi$ in Lemma~\ref{lemma:bound} is different. The proof of Lemma~\ref{lemma:bound} can be found in Appendix~\ref{appdx:proof-lemma-bound}.

\begin{theorem}
    Suppose Assumptions~\ref{assum:lipschitz}, \ref{assum:strongly-convex} holds true, and the cost functions of all agents satisfies $r$-redundancy. Assume that $\eta_t$ in (\ref{eqn:update}) satisfying $\sum_{t=0}^\infty\eta_t=\infty$ and $\sum_{t=0}^\infty\eta_t^2<\infty$, the algorithm has 
    \begin{equation}
        \lim_{t\rightarrow\infty}x^t=x^*, %x^t\xrightarrow[t\rightarrow\infty]{}x^* 
    \end{equation}
    where $x^*=\arg\min_x\sum_{i\in[n]}Q_i(x)$.
    \label{thm:exact}
\end{theorem}

\begin{proof}
\textbf{First}, we show that $\norm{\sum_{j\in S^t}\nabla Q_j(x^t)}$ is bounded for all $t$. By Assumption~\ref{assum:lipschitz}, for all $i$, $\norm{\nabla Q_i(x^t)-\nabla Q_i(x^*)}\leq\mu\norm{x^t-x^*}$.
Combining it with Lemma~\ref{lemma:minimum}, we have 
  \begin{equation}
    \norm{\nabla Q_i(x^t)}\leq\mu\norm{x^t-x^*}.
\end{equation}
By triangle inequality,
\begin{align}
    \norm{\sum_{j\in S^t}\nabla Q_j(x^t)}\leq\sum_{j\in S^t}\norm{\nabla Q_j(x^t)}\leq\mnorm{S^t}\cdot\mu\norm{x^t-x^*}.
\end{align}
Recall that $x^t\in\W$ for all $t$, where $\W$ is a compact set. There exists a $\Gamma=\max_{x\in\W}\norm{x-x^*}<\infty$, such that $\norm{x^t-x^*}\leq\Gamma$ for all $t$. Also note that $|S^t|=n-r$. Therefore, we have
\begin{align}
    \norm{\sum_{j\in S^t}\nabla Q_j(x^t)}\leq(n-r)\mu\Gamma,~\forall t.
\end{align}
Therefore, $\norm{\sum_{j\in S^t}\nabla Q_j(x^t)}$ is bounded for all $t$.

\textbf{Second}, consider the following term $\displaystyle\phi_t=\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)}$.
Recall Lemma~\ref{lemma:minimum}, $\nabla Q_j(x^*)=0$ for all $j\in[n]$. With Assumption~\ref{assum:strongly-convex}, 
\begin{align}
    \phi_t&=\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)}~=~\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)-\sum_{j\in S^t}\nabla Q_j(x^*)} \nonumber \\
        &=\mnorm{S^t}\cdot\iprod{x^t-x^*}{\nabla Q_{S^t}(x^t)-\nabla Q_{S^t}(x^*)} \geq(n-r)\gamma\norm{x^t-x^*}^2 
\end{align}
Therefore, for an arbitrary $\delta>0$, $\phi_t\geq(n-r)\gamma\delta$ so long as $\norm{x^t-x^*}\geq\delta$.

Applying Lemma~\ref{lemma:bound} with $\M=(n-r)\mu\Gamma$, $\xi=(n-r)\gamma\delta$, and $\D^*=\delta$, we obtain that for all $\delta>0$, $\lim_{t\rightarrow\infty}\norm{x^t-x^*}\leq\delta$. By the arbitrariness of $\delta$, 
$\displaystyle \lim_{t\rightarrow\infty}\norm{x^t-x^*}\leq0$. 
Since $\norm{x^t-x^*}$ is always non-negative,
$\lim_{t\rightarrow\infty}x^t=x^*$. 
\end{proof}

\subsection{Approximate Redundancy}
\label{sec:approx-redundancy}

Although the special case of $r$-redundancy discussed in the previous section allows computation of an exact minimum point of the aggregated cost functions of all agents by our algorithm, practical realization of $r$-redundancy can be difficult in the presence of \textit{noise} in real-world systems. In this section, we need to consider the general \textit{$(r,\epsilon)$-redundancy}, introduced in Definition~\ref{def:approx_redundancy}, and provide convergence analysis of our algorithm given the cost functions of agents satisfies $(r,\epsilon)$-redundancy. 

Intuitively, when $(r,\epsilon)$-redundancy is satisfied, our algorithm is guaranteed to output an approximation of the true minimum point of the aggregated cost functions of all agents. 
With $(r,\epsilon)$-redundancy among cost functions of all agents, our algorithm can output a point such that its distance to the true minimum $x^*=\arg\min_x\sum_{i\in[n]}Q_i(x)$ is bounded.

% The same as the conclusion in Section~\ref{sec:exact-redundancy} regarding the existence of a minimum point \eqref{eqn:existence-exact}, .

% With the existence assumption, we prove the following theorem on convergence with approximate redundancy condition.

\begin{theorem}
     Suppose that Assumptions~\ref{assum:lipschitz} and \ref{assum:strongly-convex} hold true, and the cost functions of all agents satisfies $(r,\epsilon)$-redundancy. 
     Assume that $\eta_t$ in (\ref{eqn:update}) satisfies $\sum_{t=0}^\infty\eta_t=\infty$ and $\sum_{t=0}^\infty\eta_t^2<\infty$.
     Let $\alpha$ and $D$ be defined as follows: $\alpha\triangleq 1-\dfrac{r}{n}\cdot\dfrac{\mu}{\gamma}>0$ and $\D\triangleq\dfrac{2r\mu}{\alpha\gamma}\epsilon$. Then, for the proposed algorithm 
    \begin{equation}
        \lim_{t\rightarrow\infty}\norm{x^t-x^*}\leq\D,%x^t\xrightarrow[t\rightarrow\infty]{}x^* 
    \end{equation}
    where $x^*=\arg\min_x\sum_{i\in[n]}Q_i(x)$.
    \label{thm:approx}
\end{theorem}

Note that Lemma~\ref{lemma:minimum} no longer holds with $(r,\epsilon)$-redundancy. 

\begin{proof}
\textbf{First}, we need to show that $\norm{\sum_{j\in S^t}\nabla Q_j(x^t)}$ is bounded for all $t$. By Assumption~\ref{assum:lipschitz}, for all $j\in[n]$, 
\begin{equation}
    \label{eqn:thm2-lip}
    \norm{\nabla Q_j(x)-\nabla Q_j(x^*)}\leq\mu\norm{x-x^*}.
\end{equation}

Let $x_S=\arg\min_x\sum_{j\in S}Q_j(x)$ be the minimum point of the aggregated cost functions of a set $S$ of $n-r$ agents, i.e., $\mnorm{S}=n-f$. Note that $\sum_{j\in S}\nabla Q_j(x_S)=0$.
By triangle inequality,
\begin{equation}
    \label{eqn:thm2-triangle}
    \norm{\sum_{j\in S}\nabla Q_j(x_S)-\sum_{j\in S}\nabla Q_j(x^*)}\leq\sum_{j\in S}\norm{\nabla Q_j(x_S)-\nabla Q_j(x^*)}.
\end{equation}
Combining~\eqref{eqn:thm2-lip} through \eqref{eqn:thm2-triangle}, %also recall $Q_S(x)=\frac{1}{\mnorm{S}}\sum_{j\in S}Q_j(x)$,
\begin{equation}
    \norm{\sum_{j\in S}\nabla Q_j(x^*)}\leq\mnorm{S}\mu\norm{x_S-x^*}.
\end{equation}
By Definition~\ref{def:approx_redundancy} of $(r,\epsilon)$-redundancy, $\norm{x_S-x^*}\leq\epsilon$.
Therefore,
\begin{equation}
    \norm{\sum_{j\in S}\nabla Q_j(x^*)}\leq\mu\epsilon (n-r).
\end{equation}

Now, consider an arbitrary agent $i\in[n]\backslash S$. Let $T=S\cup\{i\}$. Using a similar argument as above, we obtain %that with Assumption~\ref{assum:strongly-convex}, for all $x_T=\arg\min_x\sum_{j\in T}Q_j(x)$,
\begin{equation}
    \norm{\sum_{j\in T}\nabla Q_j(x^*)}\leq\mu\epsilon (n-r+1).
\end{equation}
Therefore, %by the arbitrariness of $S$ and $i$, for each agent $i\in[n]$,
\begin{align}
    \norm{\nabla Q_i(x^*)}=&\norm{\sum_{j\in T}\nabla Q_j(x^*)-\sum_{j\in S}\nabla Q_j(x^*)} \leq\norm{\sum_{j\in T}\nabla Q_j(x^*)}+\norm{\sum_{j\in S}\nabla Q_j(x^*)} \nonumber \\
        \leq&(n-r)\mu\epsilon+(n-r+1)\mu\epsilon=(2n-2r+1)\mu\epsilon. \label{eqn:apprx_gradient_bnd}
\end{align}
Note that the inequality \eqref{eqn:apprx_gradient_bnd} can be applied to any $i\in[n]$ with a suitable choice of $S$ above.\\

On the other hand, by Assumption~\ref{assum:lipschitz}, for any $x\in\mathbb{R}^d$,
\begin{equation}
    \norm{\nabla Q_i(x)-\nabla Q_i(x^*)}\leq\mu\norm{x-x^*}.
\end{equation}
By triangle inequality,
\begin{equation}
    \norm{\nabla Q_i(x)}\leq\norm{\nabla Q_i(x^*)}+\mu\norm{x-x^*}.
\end{equation}
Combining above and \eqref{eqn:apprx_gradient_bnd},
\begin{equation}
    \label{eqn:apprx_gradient_bnd_2}
    \norm{\nabla Q_i(x)}\leq(2n-2r+1)\mu\epsilon+\mu\norm{x-x^*}\leq2n\mu\epsilon+\mu\norm{x-x^*}.
\end{equation}
Recall that $x^t\in\W$ for all $t$, where $\W$ is a compact set. There exists a $\Gamma=\max_{x\in\W}\norm{x-x^*}<\infty$, such that $\norm{x^t-x^*}\leq\Gamma$ for all $t$. 
Therefore, for all $t$, 
\begin{align}
    \label{eqn:apprx_phi_t_bnd}
    \norm{\sum_{j\in S^t}\nabla Q_j(x^t)}&=\norm{\sum_{j\in S^t}\nabla Q_j(x^t)}\leq\sum_{j\in S^t}\norm{\nabla Q_j(x^t)} \nonumber \\
        &\leq\mnorm{S^t}\cdot\left(2n\mu\epsilon+\mu\norm{x^t-x^*}\right)\leq(n-r)\left(2n\mu\epsilon+\mu\Gamma\right)<\infty.
\end{align}

\textbf{Second}, consider the following term $\displaystyle\phi_t=\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)}$.
We have
\begin{align}
    \label{eqn:apprx_phi_t_1}
    \phi_t=&\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)} \nonumber \\
        =&\iprod{x^t-x^*}{\sum_{j\in S^t}\nabla Q_j(x^t)+\sum_{k\in [n]\backslash S^t}\nabla Q_k(x^t)-\sum_{k\in [n]\backslash S^t}\nabla Q_k(x^t)} \nonumber \\
        =&\iprod{x^t-x^*}{\sum_{j\in [n]}\nabla Q_j(x^t)}-\iprod{x^t-x^*}{\sum_{k\in [n]\backslash S^t}\nabla Q_k(x^t)}.
\end{align}

For the first term in \eqref{eqn:apprx_phi_t_1}, recall that $Q_S(x)=\frac{1}{\mnorm{S}}\sum_{j\in S}Q_j(x)$ for any set $S$ that satisfies $\mnorm{S}\geq n-r$. With Assumption~\ref{assum:strongly-convex}, 
\begin{align}
    \label{eqn:apprx_phi_t_1_1}
    &\iprod{x^t-x^*}{\sum_{j\in [n]}\nabla Q_j(x^t)}=\iprod{x^t-x^*}{\sum_{j\in [n]}\nabla Q_j(x^t)-\sum_{j\in [n]}\nabla Q_j(x^*)} \nonumber \\
        =&n\cdot\iprod{x^t-x^*}{\nabla Q_{[n]}(x^t)-\nabla Q_{[n]}(x^*)}\geq n\gamma\norm{x^t-x^*}^2.
\end{align}

For the second term in \eqref{eqn:apprx_phi_t_1}, by Cauchy-Schwartz inequality,
\begin{align}
    \label{eqn:apprx_phi_t_1_2}
    \iprod{x^t-x^*}{\sum_{k\in [n]\backslash S^t}\nabla Q_k(x^t)}&=\sum_{k\in [n]\backslash S^t}\iprod{x^t-x^*}{\nabla Q_k(x^t)}\nonumber \\
        &\leq\sum_{k\in [n]\backslash S^t}\norm{x^t-x^*}\cdot\norm{\nabla Q_k(x^t)}.
\end{align}

Combining \eqref{eqn:apprx_phi_t_1}, \eqref{eqn:apprx_phi_t_1_1}, and \eqref{eqn:apprx_phi_t_1_2},
\begin{equation}
    \label{eqn:apprx_phi_t_2}
    \phi_t\geq n\gamma\norm{x^t-x^*}^2-\sum_{k\in[n]\backslash S^t}\norm{x^t-x^*}\norm{\nabla Q_k(x^t)}.
\end{equation}
Substituting from \eqref{eqn:apprx_gradient_bnd_2} in above, note that $\mnorm{[n]\backslash S^t}=r$,
\begin{align}
    \label{eqn:apprx_phi_t_3}
    \phi_t&\geq n\gamma\norm{x^t-x^*}^2-\sum_{k\in[n]\backslash S^t}\norm{x^t-x^*}(2n\mu\epsilon+\mu\norm{x^t-x^*}) \nonumber \\
        &=n\gamma\norm{x^t-x^*}^2-r\norm{x^t-x^*}(2n\mu\epsilon+\mu\norm{x^t-x^*}) \nonumber \\
        &=n\gamma\left(1-\dfrac{r}{n}\cdot\dfrac{\mu}{\gamma}\right)\norm{x^t-x^*}\left(\norm{x^t-x^*}-\dfrac{2r\mu\epsilon}{\gamma\left(1-\dfrac{r}{n}\cdot\dfrac{\mu}{\gamma}\right)}\right).
\end{align}
Recall that we assume $\displaystyle\alpha=1-\dfrac{r}{n}\cdot\dfrac{\mu}{\gamma}>0$.
We have
\begin{equation}
    \phi_t\geq\alpha n\gamma\norm{x^t-x^*}\left(\norm{x^t-x^*}-\dfrac{2r\mu}{\alpha\gamma}\epsilon\right).
    \label{eqn:phi_t_final}
\end{equation}
Let $\D\triangleq\dfrac{2r\mu}{\alpha\gamma}\epsilon$. \eqref{eqn:phi_t_final} implies for an arbitrary $\delta>0$, 
\begin{equation}
    \phi_t\geq\alpha n\gamma\delta\left(D+\delta\right)>0~\textrm{ when }~\norm{x^t-x^*}\geq\D+\delta. 
\end{equation}
Therefore, by Lemma~\ref{lemma:bound}, $\lim_{t\rightarrow\infty}\norm{x^t-x^*}\leq\D$.
\end{proof}

We also offer a convergence rate analysis of our algorithm, whose proof can be found in Appendix~\ref{appdx:proof-rate}.
\begin{theorem}
    \label{thm:conv-rate}
    Suppose Assumptions~\ref{assum:lipschitz} and \ref{assum:strongly-convex} hold, and the cost functions of all agents satisfies $(r,\epsilon)$-redundancy. 
    Define $\alpha=\cfrac{\gamma}{\mu}-\cfrac{r}{n}$, $\overline{\eta}=\cfrac{2\alpha}{\mu n}$, and $A=1-(\mu n)^2\eta(\overline{\eta}-\eta)$ for some $\eta$.
    Suppose that $\eta_t=\eta$ for every iteration $t$ with $\eta\in(0,\overline{\eta})$. There exists a positive constant $R>0$, such that our algorithm satisfy the following:
    \begin{enumerate}
        \item $A\in[0,1)$, and 
        \item $\norm{x^t-x^*}^2\leq A^t\norm{x^0-x^*}+R$.
    \end{enumerate}
\end{theorem}
Theorem~\ref{thm:conv-rate} implies that the sequence of estimates $\left\{x^t\right\}$ generated by our algorithm converges \textit{linearly} to a ball centered by the true minimum $x^*$ of radius $R$.


==> experiment.tex <==
\section{Numerical experiments}
\label{sec:exp}

In this section, we present some simulation results in order to empirically demonstrate the effectiveness of our algorithm given the redundancy of cost functions. We consider two distributed linear regression problems, a special distributed optimization problem with quadratic cost functions, each corresponding to a form of redundancy in the cost functions introduced in Section \ref{sec:redundancy}.

\subsection{Experiments for exact redundancy}
\label{sub:exact-exp}
\subsubsection{Problem description}
\label{ssub:exact-problem}

In our simulations for $r$-redundancy, we select $n=6$, $d=2$, and $r=2$. Each agent $i$ ($i\in[n]$) is associated with a data point represented by an ordered pair of values $(A_i,B_i)$ where $A_i$ is a $d$-dimensional row vector, and $B_i\in\R$ as the response. Specifically, for all $i\in\{1,...,n\}$, 
\begin{equation}
    B_i=A_ix^*, \textrm{ where }x^*=\begin{pmatrix}
        1\\1
    \end{pmatrix}.
\end{equation}
The collective data, or the \textit{dataset}, is represented by an ordered pair of matrices $(A,B)$, where the $i$-th row of $A$ and $B$ are equal to $A_i$ and $B_i$, respectively. The specific values used in our simulation are as follows:
\begin{equation}
    A=\begin{pmatrix}
        1 & 0 \\
        0.8 & 0.5 \\
        0.5 & 0.8 \\
        0 & 1 \\
        -0.5 & 0.8 \\
        -0.8 & 0.5 
    \end{pmatrix}, ~ 
    B=\begin{pmatrix}
        1 \\ 1.3 \\ 1.3 \\ 1 \\ 0.3 \\ -0.3
    \end{pmatrix}.
\end{equation}
Naturally,  
\begin{equation}
    B=Ax^*.
    \label{eqn:exact-matrix-eq}
\end{equation}
Recall from linear algebra that if $A$ is full-column rank, i.e., $\rank{A}=d=2$, $x^*$ is the unique solution of \eqref{eqn:exact-matrix-eq}. Our matrix $A$ is full-column rank, therefore, $x^*$ is the unique solution.

For any non-empty set $S$ of agents, we further adopt the notations of $A_S$ and $B_S$ to represent matrices of dimensions $\mnorm{S}\times2$ and $\mnorm{S}\times1$ obtained by stacking the rows $\left\{A_i,i\in S\right\}$ and $\left\{B_i,i\in S\right\}$, respectively, in the increasing order of $i$. Observe from \eqref{eqn:exact-matrix-eq} that $B_S=A_Sx^*$. 

In this distributed optimization problem, we derive a quadratic cost function for each agent $i$ defined to be
\begin{equation}
    Q_i(x)=(B_i-A_ix)^2, ~\forall x\in\R^2.
    \label{eqn:cost-function}
\end{equation}
The aggregated cost functions of any non-empty set $S$ of agents is therefore
\begin{equation}
    \sum_{i\in S}Q_i(x)=\sum_{i\in S}\left(B_i-A_ix\right)^2=\norm{B_S-A_Sx}^2. 
    \label{eqn:aggre-cost-function}
\end{equation}
As matrix $A$ is full rank, note that $A_{[n]}=A$, $B_{[n]}=B$,
\begin{equation}
    \arg\min_{x\in\R^2}\sum_{i=1}^6Q_i(x)=\arg\min_{x\in\R^2}\norm{B_{[n]}-A_{[n]}x}^2=\left(x | B=Ax \right).
    \label{eqn:single-solution}
\end{equation}
That is, the aggregated cost functions of all agents has a unique minimum point.

\subsubsection{Properties of agents' cost functions}
\label{ssub:exact-properties}

By the definition of our dataset and the cost functions, the cost functions of all agents satisfies the $r$-redundancy property, stated in Definition~\ref{def:redundancy}. 

For each agent $i$, its cost function $Q_i(x)$ is Lipschitz continuous, i.e., Assumption~\ref{assum:lipschitz} is satisfied, with Lipschitz coefficient 
\begin{equation}
    \mu=\max_{i\in[n]}2\,\overline{v}_i,
    \label{eqn:mu}
\end{equation}
where $\overline{v}_i$ denotes the largest eigenvalue of $A_i^TA_i$. Also, the average cost function of a set $S$ agents $Q_S(x)$ is strongly convex, for any $S$ subject to $\mnorm{S}\geq n-r$, i.e., Assumption~\ref{assum:strongly-convex} is satisfied, with the strong convexity coefficient
\begin{equation}
    \gamma=\min_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}=n-f\end{subarray}}\frac{2\,\underline{v}_S}{\mnorm{S}},
    \label{eqn:gamma}
\end{equation}
where $\underline{v}_S$ is the smallest eigenvalue of $A_S^TA_S$. Derivations of \eqref{eqn:mu} and \eqref{eqn:gamma} can be found in \cite[Section 10]{gupta2019byzantine}. We calculate that for our dataset, $\mu=2$ and $\gamma=0.5166$.

\subsubsection{Simulations}
\label{ssub:exact-results}

In our experiments, we use the following parameters when implementing the algorithm. In the update rule \eqref{eqn:update}, we use the following step size
\begin{equation}
    \eta_t=\frac{0.1}{\left\lfloor t/50\right\rfloor+1}
    \label{eqn:step-size}
\end{equation}
for iterations $t=0,1,2,...$. Note that this particular step-size is diminishing, i.e., it satisfies the conditions in \eqref{eqn:diminishing}. We assume the convex compact $\W\subset\R^d$ to be a $2$-dimensional hypercube $[-1000,1000]^2$. Finally, in all executions of our experiments, we select the initial estimate $x^0=(0,0)$. 

We compare the behavior of our algorithm with the typical synchronous distributed optimization algorithm with gradient descent, where in each iteration, the server wait for all agents submitting their gradient. Our algorithm presented in Section \ref{sec:intro} is simulated based on the same synchronous optimization algorithm with randomly dropping gradients from $r$ agents in each iteration: the $r$ agents represents those whose gradients are not received by the server in each iteration. Note that in different iterations, the $r$ agents can be different. The performance of both algorithms is presented by (1) the aggregated cost functions of all agents $\sum_{i=1}^6Q_i(x^t)$ (referred to as \textit{loss}), and (2) the error of estimate $\norm{x^t-x^*}$ (referred to as \textit{distance}) for each iteration $t$. 

In both executions, we observe that the iterative estimates produced by the algorithms practically converge after 400 iterations. Thus, to measure the performance of the algorithms, we define the output of the algorithm to be $x_{\textrm{out}}=x^{500}$. The output of the two algorithms are shown in Table~\ref{tab:result-1}. We also plot performance of the algorithms for iteration $t$ ranging from 0 to 500 in these executions in Figure~\ref{fig:result-1}. 

As is shown in Table~\ref{tab:result-1} and Figure~\ref{fig:result-1}, our algorithm performs almost identical to the synchronous algorithm while tolerating $r=2$ asynchronous agents in each iteration. Both algorithms output the vector $x_{\textrm{out}}$ close enough to the true answer $x^*$ that their distance can be numerically ignored. That is to say, the estimates of our algorithm converge to the exact minimum point $x^*$, as Theorem~\ref{thm:exact} states.

\begin{table}[t]
    \centering
    \caption{\textit{\small{Output of the algorithms and corresponding errors of the estimate in exact-redundancy simulations: our algorithm in \emph{Section \ref{sec:intro}} (\emph{asynchronous}), and the typical synchronous distributed optimization algorithm (\emph{synchronous}).}}}
    \begin{tabular}{c|cc}
         & Asynchronous & Synchronous \\
        \hline
        $x_{\textrm{out}}$ & $\begin{pmatrix}.999998\\.999998\end{pmatrix}$ & $\begin{pmatrix}.999997\\.999997\end{pmatrix}$  \\
        $\dist{x^*}{x_{\textrm{out}}}$ & $2.62\times10^{-6}$ & $3.59\times10^{-6}$ 
    \end{tabular}
    \label{tab:result-1}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{optimization/async-precise-comparison-2.pdf}
    \caption{\textit{\small{Performance of the algorithms in exact-redundancy simulations. \emph{Asynchronous} (in \emph{yellow}) represents our algorithm in \emph{Section \ref{sec:intro}} while \emph{synchronous} (in \emph{blue}) represent the typical synchronous distributed optimization algorithm. The performance is presented by the \emph{losses}, i.e., $\sum_{i=1}^6Q_i(x^t)$, and \emph{distances}, i.e., $\norm{x^t-x^*}$. Note that the two algorithms has almost identical performance, hence their corresponding plots are almost coincident.}}}
    \label{fig:result-1}
\end{figure}

\subsection{Experiments for approximate redundancy}
\label{sub:approx-exp}

Similar to the exact-redundancy experiments presented in Section \ref{sub:exact-exp}, we now present a group of experiments for the approximate redundancy.

\subsubsection{Problem description}
\label{ssub:approx-problem}

In our simulations for $(r,\epsilon)$-redundancy, we also select $n=6$, $d=2$, and $r=2$. Each agent $i$ ($i\in[n]$) is associated with a data point represented by a triplet of values $(A_i, B_i, N_i)$, where $A_i$ is a $d$-dimensional row vector, $B_i\in\R$ as the response, and $N_i\in\R$ as a noise value. Specifically, for all $i\in\{1,...,n\}$,
\begin{equation}
    B_i=A_i\widehat{x}+N_i, ~\textrm{where }\widehat{x}=\begin{pmatrix}1\\1\end{pmatrix}. 
\end{equation}
The dataset is represented by a triplet of matrices $(A,B,N)$, where the $i$-th row of $A$, $B$ and $N$ are equal to $A_i$, $B_i$ and $N_i$, respectively. The specific values are as follows:
\begin{equation}
    A=\begin{pmatrix}
        1 & 0 \\
        0.8 & 0.5 \\
        0.5 & 0.8 \\
        0 & 1 \\
        -0.5 & 0.8 \\
        -0.8 & 0.5 
    \end{pmatrix}, ~ 
    B=\begin{pmatrix}
        %0.9108 \\  1.3349 \\ 1.3376 \\ 1.0033 \\ 0.2142 \\ -0.3615
        0.9666\\1.5658\\1.0297\\1.2655\\0.0239\\-0.1739
    \end{pmatrix}, ~ \text{ and }
    N=\begin{pmatrix}
        %-0.0892 \\0.0349 \\0.0376\\0.0033\\-0.0858\\-0.0615
        -0.0334\\0.2658\\-0.2703\\0.2655\\-0.2761\\0.1261
    \end{pmatrix}.
\end{equation}
Also note that
\begin{equation}
    B=A\,\widehat{x}+N.
\end{equation}
Recall from Section \ref{ssub:exact-problem} that $A$ is full-column rank, and therefore, the following equation has a unique solution $x^*$:
\begin{equation}
    B=Ax.
\end{equation}
It can be calculated that $x^*=\begin{pmatrix}1.0293\\1.0087\end{pmatrix}$. Similarly, for any set $S$ of agents ($\mnorm{S}\geq n-r=6-2=4$), it can be verified that the matrix $A_S$ is full-column rank, i.e., $\rank{A_S}=d=2$. Therefore, for any $S$ ($\mnorm{S}\geq4$), there exists $x_S$ being the unique solution to the following equation:
\begin{equation}
    B_S=A_Sx.
\end{equation}

We define the quadratic cost function of agents and the aggregated cost function the same way as stated in equations \eqref{eqn:cost-function}, \eqref{eqn:aggre-cost-function}. By the same reasoning in \eqref{eqn:single-solution}, $x^*$ is the unique minimum point of the aggregated cost functions of all agents.

\subsubsection{Properties of agents' cost functions}
\label{ssub:approx-properties}

The cost functions of all agents satisfy the $(r,\epsilon)$-redundancy property, stated in Definition~\ref{def:approx_redundancy}, with the approximation coefficient 
\begin{equation}
    \epsilon = \max_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}\geq n-f\end{subarray}}\dist{x_S}{x^*} = \max_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}\geq 4\end{subarray}}\norm{x_S-x^*}.
\end{equation}
For our dataset, $\epsilon=0.3163$.

Recall the ways of computing $\mu$ and $\gamma$ state in \eqref{eqn:mu} and \eqref{eqn:gamma}, respectively. 
For each agent $i$, its cost function $Q_i(x)$ is Lipschitz continuous, i.e., Assumption~\ref{assum:lipschitz} is satisfied, with Lipschitz coefficient
$\mu = 2$. The average cost function of a set $S$ of agents $Q_S(x)$ is strongly convex, for any $S$ subject to $|S|\geq n-r$, i.e., Assumption~\ref{assum:strongly-convex} is satisfied, with the strong convexity coefficient $\gamma = 0.5166$. Note that since the matrix $A$ is the same as in Section~\ref{ssub:exact-properties}, the values of $\mu$ and $\gamma$ remain the same as well. 

\subsubsection{Simulations}
\label{ssub:approx-results}

In our experiments for approximate redundancy, we use the same parameters as stated in Section~\ref{ssub:exact-results}, namely the step sizes $\eta_t$, the convex compact set $\W$, and the initial estimate $x^0$. We also compare the performance of our algorithm and the typical synchronous distributed optimization algorithm. The $r$ agents whose gradients are not received by the server in each iteration is simulated in the same way as stated in Section~\ref{ssub:exact-results}. 

In the experiment of our algorithm, the iterative estimates become fluctuating within a small area after 400 iterations. The estimates of the synchronous algorithm also converge after 400 iterations. Thus, to measure the performance of the algorithms, we define the output of the algorithm to be $x_{\textrm{out}}=x^{500}$. The output of the two algorithms are shown in Table~\ref{tab:result-2}. We also plot performance of the algorithms for iteration $t$ ranging from 0 to 500 in these executions in Figure~\ref{fig:result-2}, along with details of $t$ ranging from 10 to 500 shown in Figure~\ref{fig:result-2-detail}. 

As is shown in Table~\ref{tab:result-2} and Figures~\ref{fig:result-2} and \ref{fig:result-2-detail}, although our algorithm cannot converge to a certain point near the exact minimum point $x^*$ as the synchronous algorithm does, its estimates are asymptotically bounded within distance $\epsilon$ to $x^*$, as Theorem~\ref{thm:approx} states. In this simulation, the distance is even smaller than $\epsilon$ indicates. 

\begin{table}[t]
    \centering
    \caption{\textit{\small{Output of the algorithms and corresponding errors of the estimate in approximate-redundancy simulations: our algorithm in \emph{Section \ref{sec:intro}} (\emph{asynchronous}), and the typical synchronous distributed optimization algorithm (\emph{synchronous}).}}}
    \begin{tabular}{c|cc}
         & Asynchronous & Synchronous \\
        \hline
        $x_{\textrm{out}}$ & $\begin{pmatrix}1.0260\\1.0049\end{pmatrix}$ & $\begin{pmatrix}1.0293\\1.0087\end{pmatrix}$  \\
        $\dist{x^*}{x_{\textrm{out}}}$ & $4.18\times10^{-3}$ & $6.24\times10^{-6}$ 
    \end{tabular}
    \label{tab:result-2}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{optimization/async-apprx2-comparison-2.pdf}
    \caption{\textit{\small{Performance of the algorithms in approximate-redundancy simulations. \emph{Asynchronous} (in \emph{yellow}) represents our algorithm in \emph{Section \ref{sec:intro}} while \emph{synchronous} (in \emph{blue}) represent the typical synchronous distributed optimization algorithm. The performance is presented by the \emph{losses}, i.e., $\sum_{i=1}^6Q_i(x^t)$, and \emph{distances}, i.e., $\norm{x^t-x^*}$. Note that the two algorithms has almost identical performance, hence their corresponding plots are almost coincident.}}}
    \label{fig:result-2}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.62\textwidth]{optimization/async-apprx2-comparison-2-details.pdf}
    \caption{\textit{\small{Performance of the algorithms in approximate-redundancy simulations, magnified for the iterations $t$ ranging from 10 to 500. The meaning of axes and plots are the same as in Figure~\ref{fig:result-2}. The horizontal line in \emph{red} marks the value of $\epsilon$.}}}
    \label{fig:result-2-detail}
\end{figure}


==> experiment_v2.tex <==
\section{Experiments}
\label{sec:exp}

In this section, we present some simulation results to empirically demonstrate the effectiveness of our algorithm given the redundancy of cost functions. In Section \ref{sub:approx-exp}, we present a numerical experiment with cost functions satisfying the assumptions required by our theoretical results. Then in Section~\ref{sec:exp-learning}, we present a group of experiments on machine learning tasks to demonstrate the effectiveness of our algorithm in real-world scenario.

\subsection{Numerical experiments}
\label{sub:approx-exp}

We present a quadratic optimization problem satisfying $(r,\epsilon)$-redundancy and assumptions required in Theorem~\ref{thm:approx}, and performance of our algorithm on solving this problem.

\subsubsection{Problem description}
\label{ssub:approx-problem}

In our simulations for $(r,\epsilon)$-redundancy, we select $n=6$, $d=2$, and $r=2$. Each agent $i$ ($i\in[n]$) is associated with a data point represented by a triplet of values $(A_i, B_i, N_i)$, where $A_i$ is a $d$-dimensional row vector, $B_i\in\R$ as the response, and $N_i\in\R$ as a noise value. Specifically, for all $i\in\{1,...,n\}$,
\begin{equation}
    B_i=A_i\widehat{x}+N_i, ~\textrm{where }\widehat{x}=\begin{pmatrix}1\\1\end{pmatrix}. 
\end{equation}
The collective data, or the \textit{dataset}, is represented by a triplet of matrices $(A,B,N)$, where the $i$-th row of $A$, $B$ and $N$ are equal to $A_i$, $B_i$ and $N_i$, respectively. The specific values are as follows:
\begin{equation}
    A=\begin{pmatrix}
        1 & 0 \\
        0.8 & 0.5 \\
        0.5 & 0.8 \\
        0 & 1 \\
        -0.5 & 0.8 \\
        -0.8 & 0.5 
    \end{pmatrix}, ~ 
    B=\begin{pmatrix}
        %0.9108 \\  1.3349 \\ 1.3376 \\ 1.0033 \\ 0.2142 \\ -0.3615
        0.9666\\1.5658\\1.0297\\1.2655\\0.0239\\-0.1739
    \end{pmatrix}, ~ \text{ and }
    N=\begin{pmatrix}
        %-0.0892 \\0.0349 \\0.0376\\0.0033\\-0.0858\\-0.0615
        -0.0334\\0.2658\\-0.2703\\0.2655\\-0.2761\\0.1261
    \end{pmatrix}.
\end{equation}
Also note that
\begin{equation}
    B=A\,\widehat{x}+N.
\end{equation}
Recall from linear algebra that if $A$ is full-column rank, i.e., $\rank{A}=d=2$, the following equation has a unique solution $x^*$:
\begin{equation}
    \label{eqn:approx-matrix-eq}
    B=Ax.
\end{equation}
Our matrix $A$ is full-column rank, therefore, $x^*$ is the unique solution. \eqref{eqn:approx-matrix-eq} can be solved that $x^*=\begin{pmatrix}1.0293\\1.0087\end{pmatrix}$. The goal of the optimization problem is to numerically solve \eqref{eqn:approx-matrix-eq}.

For any non-empty set $S$ of agents, we further adopt the notations of $A_S$ and $B_S$ to represent matrices of dimensions $\mnorm{S}\times2$ and $\mnorm{S}\times1$ obtained by stacking the rows $\left\{A_i,i\in S\right\}$ and $\left\{B_i,i\in S\right\}$, respectively, in the increasing order of $i$. %Observe from \eqref{eqn:approx-matrix-eq} that $B_S=A_Sx^*$. 
In this distributed optimization problem, we derive a quadratic cost function for each agent $i$ defined to be
\begin{equation}
    Q_i(x)=(B_i-A_ix)^2, ~\forall x\in\R^2.
    \label{eqn:cost-function}
\end{equation}
The aggregated cost functions of any non-empty set $S$ of agents is therefore
\begin{equation}
    \sum_{i\in S}Q_i(x)=\sum_{i\in S}\left(B_i-A_ix\right)^2=\norm{B_S-A_Sx}^2. 
    \label{eqn:aggre-cost-function}
\end{equation}
As matrix $A$ is full rank, note that $A_{[n]}=A$, $B_{[n]}=B$,
\begin{equation}
    \arg\min_{x\in\R^2}\sum_{i=1}^6Q_i(x)=\arg\min_{x\in\R^2}\norm{B_{[n]}-A_{[n]}x}^2=\left(x | B=Ax \right).
    \label{eqn:single-solution}
\end{equation}
That is, the aggregated cost functions of all agents has a unique minimum point $x^*$.

Similarly, for any set $S$ of agents ($\mnorm{S}\geq n-r=6-2=4$), it can be verified that the matrix $A_S$ is full-column rank, i.e., $\rank{A_S}=d=2$. Therefore, for any $S$ ($\mnorm{S}\geq4$), there exists $x_S$ being the unique solution to the following equation:
\begin{equation}
    B_S=A_Sx.
\end{equation}

\subsubsection{Properties of agents' cost functions}
\label{ssub:approx-properties}

The cost functions of all agents satisfy the $(r,\epsilon)$-redundancy property, stated in Definition~\ref{def:approx_redundancy}, with the approximation coefficient 
\begin{equation}
    \epsilon = \max_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}\geq n-f\end{subarray}}\dist{x_S}{x^*} = \max_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}\geq 4\end{subarray}}\norm{x_S-x^*}.
\end{equation}
For our dataset, $\epsilon=0.3163$.

For each agent $i$, its cost function $Q_i(x)$ is Lipschitz continuous, i.e., Assumption~\ref{assum:lipschitz} is satisfied, with Lipschitz coefficient 
\begin{equation}
    \mu=\max_{i\in[n]}2\,\overline{v}_i,
    \label{eqn:mu}
\end{equation}
where $\overline{v}_i$ denotes the largest eigenvalue of $A_i^TA_i$. Also, the average cost function of a set $S$ agents $Q_S(x)$ is strongly convex, for any $S$ subject to $\mnorm{S}\geq n-r$, i.e., Assumption~\ref{assum:strongly-convex} is satisfied, with the strong convexity coefficient
\begin{equation}
    \gamma=\min_{\begin{subarray}{c}S\subseteq[n]\\\mnorm{S}=n-f\end{subarray}}\frac{2\,\underline{v}_S}{\mnorm{S}},
    \label{eqn:gamma}
\end{equation}
where $\underline{v}_S$ is the smallest eigenvalue of $A_S^TA_S$. Derivations of \eqref{eqn:mu} and \eqref{eqn:gamma} can be found in \cite[Section 10]{gupta2019byzantine}. We calculate that for our dataset, $\mu=2$ and $\gamma=0.5166$.

%Recall the ways of computing $\mu$ and $\gamma$ state in \eqref{eqn:mu} and \eqref{eqn:gamma}, respectively. 
%For each agent $i$, its cost function $Q_i(x)$ is Lipschitz continuous, i.e., Assumption~\ref{assum:lipschitz} is satisfied, with Lipschitz coefficient
%$\mu = 2$. The average cost function of a set $S$ of agents $Q_S(x)$ is strongly convex, for any $S$ subject to $|S|\geq n-r$, i.e., Assumption~\ref{assum:strongly-convex} is satisfied, with the strong convexity coefficient $\gamma = 0.5166$. Note that since the matrix $A$ is the same as in Section~\ref{ssub:exact-properties}, the values of $\mu$ and $\gamma$ remain the same as well. 

\subsubsection{Simulations}
\label{ssub:approx-results}

In our experiments, we use the following parameters when implementing the algorithm. In the update rule \eqref{eqn:update}, we use the following step size
\begin{equation}
    \eta_t=\frac{0.1}{\left\lfloor t/50\right\rfloor+1}
    \label{eqn:step-size}
\end{equation}
for iterations $t=0,1,2,...$. Note that this particular step-size is diminishing, i.e., it satisfies the conditions in \eqref{eqn:diminishing}. We assume the convex compact $\W\subset\R^d$ to be a $2$-dimensional hypercube $[-1000,1000]^2$. Finally, in all executions of our experiments, we use the initial estimate $x^0=(0,0)$. 

We compare the behavior of our algorithm with the typical synchronous distributed optimization algorithm with gradient descent, where in each iteration, the server wait for all agents submitting their gradient. Our algorithm presented in Section \ref{sec:intro} is simulated based on the same synchronous optimization algorithm with randomly dropping gradients from $r$ agents in each iteration, representing those whose gradients are not received by the server in each iteration. Note that in different iterations, the $r$ agents can be different. The performance of both algorithms is presented by (1) the aggregated cost functions of all agents $\sum_{i=1}^6Q_i(x^t)$ (referred to as \textit{loss}), and (2) the error of estimate $\norm{x^t-x^*}$ (referred to as \textit{distance}) for each iteration $t$. 

In the experiment of our algorithm, the iterative estimates become fluctuating within a small area after 400 iterations. The estimates of the synchronous algorithm also converge after 400 iterations. Thus, to measure the performance of the algorithms, we define the output of the algorithm to be $x_{\textrm{out}}=x^{500}$. The output of the two algorithms are shown in Table~\ref{tab:result-2}. We also plot performance of the algorithms for iteration $t$ ranging from 0 to 500 in these executions in Figure~\ref{fig:result-2}, along with details of $t$ ranging from 10 to 500 shown in Figure~\ref{fig:result-2-detail}.  

As is shown in Table~\ref{tab:result-2} and Figures~\ref{fig:result-2} and \ref{fig:result-2-detail}, although our algorithm cannot converge to a certain point near the exact minimum point $x^*$ as the synchronous algorithm does, its estimates are asymptotically bounded within distance $\epsilon$ to $x^*$, as Theorem~\ref{thm:approx} states. In our simulation, the distance is actually much smaller than the theoretical bound $\epsilon$. 

\begin{table}[t]
    \centering
    \caption{\textit{\small{Output of the algorithms and corresponding errors of the estimate in approximate-redundancy simulations: our algorithm in \emph{Section \ref{sec:intro}} (\emph{asynchronous}), and the typical synchronous distributed optimization algorithm (\emph{synchronous}).}}}
    \begin{tabular}{c|cc}
         & Asynchronous & Synchronous \\
        \hline
        $x_{\textrm{out}}$ & $\begin{pmatrix}1.0260\\1.0049\end{pmatrix}$ & $\begin{pmatrix}1.0293\\1.0087\end{pmatrix}$  \\
        $\dist{x^*}{x_{\textrm{out}}}$ & $4.18\times10^{-3}$ & $6.24\times10^{-6}$ 
    \end{tabular}
    \label{tab:result-2}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{optimization/async-apprx2-comparison-2.pdf}
    \caption{\textit{\small{Performance of the algorithms in approximate-redundancy simulations. \emph{Asynchronous} (in \emph{yellow}) represents our algorithm in \emph{Section \ref{sec:intro}} while \emph{synchronous} (in \emph{blue}) represent the typical synchronous distributed optimization algorithm. The performance is presented by the \emph{losses}, i.e., $\sum_{i=1}^6Q_i(x^t)$, and \emph{distances}, i.e., $\norm{x^t-x^*}$. Note that the two algorithms has almost identical performance, hence their corresponding plots are almost coincident.}}}
    \label{fig:result-2}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.62\textwidth]{optimization/async-apprx2-comparison-2-details.pdf}
    \caption{\textit{\small{Performance of the algorithms in approximate-redundancy simulations, magnified for the iterations $t$ ranging from 10 to 500. The meaning of axes and plots are the same as in Figure~\ref{fig:result-2}. The horizontal line in \emph{red} marks the value of $\epsilon$.}}}
    \label{fig:result-2-detail}
\end{figure}



